Translation Error Detection as Rationale Extraction

Recent Quality Estimation (QE) models based on multilingual pre-trained representations have achieved very competitive results when predicting the overall quality of translated sentences. Predicting translation errors, i.e. detecting specifically which words are incorrect, is a more challenging task, especially with limited amounts of training data. We hypothesize that, not unlike humans, successful QE models rely on translation errors to predict overall sentence quality. By exploring a set of feature attribution methods that assign relevance scores to the inputs to explain model predictions, we study the behaviour of state-of-the-art sentence-level QE models and show that explanations (i.e. rationales) extracted from these models can indeed be used to detect translation errors. We therefore (i) introduce a novel semi-supervised method for word-level QE and (ii) propose to use the QE task as a new benchmark for evaluating the plausibility of feature attribution, i.e. how interpretable model explanations are to humans.

==> tables/performace_mlqe.tex <==
\begin{table}[ht]
\begin{center}
%\small
\footnotesize
\begin{tabular}{l c c c c} 
\toprule 
{\bf Method} & {\bf AUC }& {\bf AUPRC} &{\bf A@1} &{\bf R@X} \\ 
\midrule
Info. Bottleneck & 0.61 & 0.60 & 0.69 & \\
Gradients & 0.67 & 0.64 & 0.73 & 0.55 \\
Attention & 0.65 & 0.58 & 0.52 & \\
LIME & 0.60 & 0.59 & & \\
\midrule
Glassbox QE & 0.68 & 0.61 & 0.62 & 0.51 \\
MicroTransQuest & 0.82 & 0.78 & 0.87 & 0.67 \\
\midrule
Random & 0.50 & 0.38 & 0.42 & 0.38\\
\bottomrule
\end{tabular}
\end{center}
\caption{AUC/AUPRC scores, as well as accuracy at top-1 (A@1) and recall at top-X (R@X) for different rationale extraction methods on the Estonian-English MLQE-PE dataset. \note{This is for XLM-R-base model.}}
\label{tab:performance_mlqe}
\end{table}

==> tables/performace_toy.tex <==
\begin{table}[ht]
\begin{center}
%\small
\footnotesize
\begin{tabular}{l  c c c c } 
\toprule 
{\bf Method} & {\bf AUC }& {\bf AP} &{\bf A@1} &{\bf R@X} \\ 
\midrule
Information Bottleneck & 0.77 & 0.42 & 0.64 & 0.50 \\
LIME & 0.78 & 0.54 & & \\
\midrule
Random & 0.50 & 0.12 & 0.13 & 0.11\\
\bottomrule
\end{tabular}
\end{center}
\caption{Performance of different rationale extraction methods on the toy dataset.}
\label{tab:performance_toy}
\end{table}
